Real-time Geo-localization Using Satellite Imagery and Topography for Unmanned Aerial Vehicles

The capabilities of autonomous flight with unmanned aerial vehicles (UAVs) have significantly increased in recent times. However, basic problems such as fast and robust geo-localization in GPS-denied environments still remain unsolved. Existing research has primarily concentrated on improving the accuracy of localization at the cost of long and varying computation time in various situations, which often necessitates the use of powerful ground station machines. In order to make image-based geo-localization online and pragmatic for lightweight embedded systems on UAVs, we propose a framework that is reliable in changing scenes, flexible about computing resource allocation and adaptable to common camera placements. The framework is comprised of two stages: offline database preparation and online inference. At the first stage, color images and depth maps are rendered as seen from potential vehicle poses quantized over the satellite and topography maps of anticipated flying areas. A database is then populated with the global and local descriptors of the rendered images. At the second stage, for each captured real-world query image, top global matches are retrieved from the database and the vehicle pose is further refined via local descriptor matching. We present field experiments of image-based localization on two different UAV platforms to validate our results.

==> reference_old.tex <==
@INPROCEEDINGS{conte2008integrated,
  title={An integrated UAV navigation system based on aerial image matching},
  author={Conte, Gianpaolo and Doherty, Patrick},
  booktitle={IEEE Aerospace Conference},
  pages={1--10},
  year={2008},
}

@article{hinzmann2020deep,
  title={Deep UAV Localization with Reference View Rendering},
  author={Hinzmann, Timo and Siegwart, Roland},
  journal={arXiv preprint arXiv:2008.04619},
  year={2020}
}

@INPROCEEDINGS{patel2020visual,
  title={Visual localization with google earth images for robust global pose estimation of UAVs},
  author={Patel, Bhavit and Barfoot, Timothy D and Schoellig, Angela P},
  booktitle={IEEE International Conference on Robotics and Automation},
  pages={6491--6497},
  year={2020},
}

@INPROCEEDINGS{yol2014vision,
  title={Vision-based absolute localization for unmanned aerial vehicles},
  author={Yol, Aurelien and Delabarre, Bertrand and Dame, Amaury and Dartois, Jean-Emile and Marchand, Eric},
  booktitle={IEEE International Conference on Intelligent Robots and Systems},
  pages={3429--3434},
  year={2014},
}

@INPROCEEDINGS{goforth2019gps,
  title={GPS-denied UAV localization using pre-existing satellite imagery},
  author={Goforth, Hunter and Lucey, Simon},
  booktitle={IEEE International Conference on Robotics and Automation},
  pages={2974--2980},
  year={2019},
}

@INPROCEEDINGS{shetty2019uav,
  title={Uav pose estimation using cross-view geolocalization with satellite imagery},
  author={Shetty, Akshay and Gao, Grace Xingxin},
  booktitle={IEEE International Conference on Robotics and Automation},
  pages={1827--1833},
  year={2019},
}

@INPROCEEDINGS{wu2008image,
  title={Image localization in satellite imagery with feature-based indexing},
  author={Wu, Changchang and Fraundorfer, Friedrich and Frahm, Jan-Michael and Snoeyink, Jack and Pollefeys, Marc},
  booktitle={ISPRS Congress: Technical Commission III},
  volume={37},
  pages={197--202},
  year={2008},
}

@article{bianchi2021uav,
  title={UAV Localization Using Autoencoded Satellite Images},
  author={Bianchi, Mollie and Barfoot, Timothy D},
  journal={IEEE Robotics and Automation Letters},
  volume={6},
  number={2},
  pages={1761--1768},
  year={2021},
  publisher={IEEE}
}

@article{lowe2004distinctive,
  title={Distinctive image features from scale-invariant keypoints},
  author={Lowe, David G},
  journal={International journal of computer vision},
  volume={60},
  number={2},
  pages={91--110},
  year={2004},
  publisher={Springer}
}

@INPROCEEDINGS{viswanathan2014vision,
  title={Vision based robot localization by ground to satellite matching in GPS-denied situations},
  author={Viswanathan, Anirudh and Pires, Bernardo R and Huber, Daniel},
  booktitle={IEEE International Conference on Intelligent Robots and Systems},
  pages={192--198},
  year={2014},
}

@article{hu2020image,
  title={Image-based geo-localization using satellite imagery},
  author={Hu, Sixing and Lee, Gim Hee},
  journal={International Journal of Computer Vision},
  volume={128},
  number={5},
  pages={1205--1219},
  year={2020},
  publisher={Springer}
}

@INPROCEEDINGS{hu2018cvm,
  title={Cvm-net: Cross-view matching network for image-based ground-to-aerial geo-localization},
  author={Hu, Sixing and Feng, Mengdan and Nguyen, Rang MH and Lee, Gim Hee},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition},
  pages={7258--7267},
  year={2018}
}

@INPROCEEDINGS{tian2017cross,
  title={Cross-view image matching for geo-localization in urban environments},
  author={Tian, Yicong and Chen, Chen and Shah, Mubarak},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3608--3616},
  year={2017}
}

@INPROCEEDINGS{sarlin2019coarse,
  title={From coarse to fine: Robust hierarchical localization at large scale},
  author={Sarlin, Paul-Edouard and Cadena, Cesar and Siegwart, Roland and Dymczyk, Marcin},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition},
  pages={12716--12725},
  year={2019}
}

@INPROCEEDINGS{bay2006surf,
  title={Surf: Speeded up robust features},
  author={Bay, Herbert and Tuytelaars, Tinne and Van Gool, Luc},
  booktitle={European conference on computer vision},
  pages={404--417},
  year={2006},
  organization={Springer}
}

@INPROCEEDINGS{arandjelovic2016netvlad,
  title={NetVLAD: CNN architecture for weakly supervised place recognition},
  author={Arandjelovic, Relja and Gronat, Petr and Torii, Akihiko and Pajdla, Tomas and Sivic, Josef},
  booktitle={IEEE conference on computer vision and pattern recognition},
  pages={5297--5307},
  year={2016}
}

@INPROCEEDINGS{detone2018superpoint,
  title={Superpoint: Self-supervised interest point detection and description},
  author={DeTone, Daniel and Malisiewicz, Tomasz and Rabinovich, Andrew},
  booktitle={IEEE conference on computer vision and pattern recognition workshops},
  pages={224--236},
  year={2018}
}

@INPROCEEDINGS{sandler2018mobilenetv2,
  title={Mobilenetv2: Inverted residuals and linear bottlenecks},
  author={Sandler, Mark and Howard, Andrew and Zhu, Menglong and Zhmoginov, Andrey and Chen, Liang-Chieh},
  booktitle={IEEE conference on computer vision and pattern recognition},
  pages={4510--4520},
  year={2018}
}

@INPROCEEDINGS{sarlin2020superglue,
  title={Superglue: Learning feature matching with graph neural networks},
  author={Sarlin, Paul-Edouard and DeTone, Daniel and Malisiewicz, Tomasz and Rabinovich, Andrew},
  booktitle={IEEE conference on computer vision and pattern recognition},
  pages={4938--4947},
  year={2020}
}

@inproceedings{sarlin2018leveraging,
  title={Leveraging deep visual descriptors for hierarchical efficient localization},
  author={Sarlin, Paul-Edouard and Debraine, Fr{\'e}d{\'e}ric and Dymczyk, Marcin and Siegwart, Roland and Cadena, Cesar},
  booktitle={Conference on Robot Learning},
  pages={456--465},
  year={2018},
  organization={PMLR}
}

@misc{retroplasma2021,
  author = {Andrian and Arnold, Fabio and LexSong and stone and Sari, Cihan and Cameron},
  title = {earth-reverse-engineering},
  year = {2021},
  publisher = {GitHub},
  journal = {GitHub repository},
  howpublished = {\url{https://github.com/retroplasma/earth-reverse-engineering}},
  commit = {35af10d0e1a133dc217d63c59545a917f4e5fc3f}
}

